Refining Labelled Systems for Modal and Constructive Logics with Applications

This thesis introduces the "method of structural refinement", which serves as a means of transforming the relational semantics of a modal and/or constructive logic into an 'economical' proof system by connecting two proof-theoretic paradigms: labelled and nested sequent calculi. The formalism of labelled sequents has been successful in that cut-free calculi in possession of desirable proof-theoretic properties can be automatically generated for large classes of logics. Despite these qualities, labelled systems make use of a complicated syntax that explicitly incorporates the semantics of the associated logic, and such systems typically violate the subformula property to a high degree. By contrast, nested sequent calculi employ a simpler syntax and adhere to a strict reading of the subformula property, making such systems useful in the design of automated reasoning algorithms. However, the downside of the nested sequent paradigm is that a general theory concerning the automated construction of such calculi (as in the labelled setting) is essentially absent, meaning that the construction of nested systems and the confirmation of their properties is usually done on a case-by-case basis. The refinement method connects both paradigms in a fruitful way, by transforming labelled systems into nested (or, refined labelled) systems with the properties of the former preserved throughout the transformation process. To demonstrate the method of refinement and some of its applications, we consider grammar logics, first-order intuitionistic logics, and deontic STIT logics. The introduced refined labelled calculi will be used to provide the first proof-search algorithms for deontic STIT logics. Furthermore, we employ our refined labelled calculi for grammar logics to show that every logic in the class possesses the effective Lyndon interpolation property.

==> Old Files/EXTRA-SEC-Prelim-GramLog.tex <==
%Certain semantic (e.g. \dfn~\ref{def:generalized-relations-kms} below) and syntactic notions (e.g. \dfn~\ref{def:string-relations-kms} in \sect~\ref{sec:lab-calc-kms}) depend on \emph{strings} defined over $\albet$ with associated operations. We define such objects and operations below:

%\begin{definition} We let $\cdot$ to represent the usual \emph{concatenation} operation and $\varepsilon$ represent the \emph{empty string}. The set $\albet^{*}$ of \emph{strings over $\albet$} is defined to be the smallest set of strings such that 
%\begin{itemize}
%\item[$\li$] $\albet \cup \{\varepsilon\} \subseteq \albet^{*}$;

%\item[$\li$] if $\stra, \strb \in \albet^{*}$, then $\stra \strb \in \albet^{*}$. 
%\end{itemize}
%Moreover, we extend the converse operation to strings as follows:
%\begin{itemize}
%\item[$\li$] $\overline{\varepsilon} := \varepsilon$;

%\item[$\li$] if $\stra = a_{1} \cdots a_{n}$, then $\overline{\stra} := \overline{a}_{n} \cdots \overline{a}_{1}$.
%\end{itemize}
%\end{definition}

%$\albet \cup \{\varepsilon\} \subseteq \albet^{*}$, and (ii) if $\stra, \strb \in \albet^{*}$, then $\stra \strb \in \albet^{*}$. As usual, $\varepsilon$ denotes the \emph{empty string}. Moreover, we extend the converse operation to strings as follows: (i) $\overline{\varepsilon} := \varepsilon$, (ii) if $\stra = a_{1} \cdots a_{n}$, then $\overline{\stra} := \overline{a}_{n} \cdots \overline{a}_{1}$.

%We use $\stra, \strb, \strc$, etc. to denote \emph{strings} in the set $\albet^{*}$, which is defined to be the smallest set of strings such that (i) $\albet \cup \{\varepsilon\} \subseteq \albet^{*}$, and (ii) if $\stra, \strb \in \albet^{*}$, then $\stra \strb \in \albet^{*}$. As usual, $\varepsilon$ denotes the \emph{empty string}. Moreover, we extend the converse operation to strings as follows: (i) $\overline{\varepsilon} := \varepsilon$, (ii) if $\stra = a_{1} \cdots a_{n}$, then $\overline{\stra} := \overline{a}_{n} \cdots \overline{a}_{1}$.

==> Old Files/SEC-LabCalc-SubBiInt-FO.tex <==

{\color{blue} Must consider closure condition. (2) DONT FORGET NED RULE!!! (nonempty domain)}

We define our labelled sequents to be syntactic objects of the form $L_{1} \Rightarrow L_{2}$ where $L_{1}$ and $L_{2}$ are formulae defined via the BNF grammar below:
\begin{center}
\begin{tabular}{c @{\hskip 2em} c}
$L_{1} ::= w : A \ | \ w \leq u \ | \ L_{1},L_{1}$

&

$L_{2} ::= w : A \ | \ L_{2},L_{2}$
\end{tabular}
\end{center}
\begin{center}
\begin{tabular}{c @{\hskip 2em} c}
$L_{1} ::= w : A \ | \ \unda \in D_{w} \ | \ w \leq u \ | \ L_{1},L_{1}$

&

$L_{2} ::= w : A \ | \ L_{2},L_{2}$
\end{tabular}
\end{center}
where $A$ is in the language $\langsbifo$, $\unda$ is among a denumerable set of \emph{parameters} $\{\unda, \undb, \undc, \ldots\}$, and $w$ is among a denumerable set of labels $\{w, u, v, \ldots \}$. We refer to formulae of the forms $w \leq u$ and $\unda \in D_{w}$ as \emph{relational atoms} (with formulae of the form $\unda \in D_{w}$ sometimes referred to as \emph{domain atoms}, more specifically) and refer to formulae of the form $w : A$ as \emph{labelled formulae}. Due to the two types of formulae occurring in a labelled sequent, we often use $\R$ to denote relational atoms, and $\Gamma$ and $\Delta$ to denote labelled formulae, thus distinguishing between the two. Labelled sequents are therefore written in a general form as $\R, \Gamma \Rightarrow \Delta$. Moreover, we take the comma operator to be commutative and associative; for example, we identify the labelled sequent $w \leq u, w : A, \unda \in D_{w} \sar u :B, v : C$ with $\unda \in D_{w}, w \leq u, w : A \sar v : C, u :B$. This interpretation of comma lets us view $\R, \Gamma$ and $\Delta$ as multisets. Also, we allow for empty antecedents and succedents in both our labelled and nested sequents.

We syntactically distinguish between \emph{bound variables} $\{x, y, z, \ldots\}$ and \emph{free variables}, which are replaced with \emph{parameters} $\{\unda, \undb, \undc, \ldots\}$, to avoid clashes between the two categories (cf.~\cite[Sect.~8]{Fit14}). Therefore, instead of using formulae directly from the first-order language, we use formulae from the first-order language where each freely occurring variable $x$ has been replaced by a distinct parameter $\unda$. For example, we would make use of the labelled formula $w : (\forall x) p(\unda,x) \lor q(\unda,\undb)$ instead of $w : (\forall x) p(y,x) \lor q(y,z)$ in a first-order labelled sequent. For a formula $A \in \langsbifo$, we write $A(\unda/x)$ to mean the formula that results from substituting the parameter $\unda$ for all occurrences of the free variable $x$ in $A$. Last, we use the notation $A(\unda_{0}, \ldots, \unda_{n})$, with $n \in \mathbb{N}$, to denote that the parameters $\unda_{0}, \ldots, \unda_{n}$ are all parameters occurring in the formula $A$. We write $A(\vec{\unda})$ as shorthand for $A(\unda_{0}, \ldots, \unda_{n})$ and $\vec{\unda} \in D_{w}$ as shorthand for $\unda_{0} \in D_{w}, \ldots, \unda_{n} \in D_{w}$. The base labelled calculi $\mathsf{G3L}$ and $\mathsf{G3Q}$ are given in Fig.~\ref{fig:base-calc-lab}.


\begin{figure}
\noindent\hrule




\begin{center}
\begin{tabular}{c c}


&

\AxiomC{}
\RightLabel{$\idfo$}
\UnaryInfC{$\R, \vec{\unda} \in D_{w}, w :p(\vec{\unda}),\Gamma \Rightarrow \Delta, w :p(\vec{\unda})$}
\DisplayProof
\end{tabular}
\end{center}

\begin{center}
\resizebox{\columnwidth}{!}{
\begin{tabular}{c c} % @{\hskip 1em} c}

\AxiomC{$\R, w \leq v, \unda \in D_{v}, \Gamma \Rightarrow \Delta, v : A(\unda/x)$}
\RightLabel{$\allr^{\dag_{2}}$}
\UnaryInfC{$\R, \Gamma \Rightarrow \Delta, w : \forall x A$}
\DisplayProof

&

\AxiomC{$\R, \unda \in D_{w}, \Gamma \Rightarrow \Delta, w: A(\unda/x), w: \exists x A$}
\RightLabel{$\existsr$}
\UnaryInfC{$\R, \unda \in D_{w}, \Gamma \Rightarrow \Delta, w: \exists x A$}
\DisplayProof

\end{tabular}
}
\end{center}

\begin{center}
\resizebox{\columnwidth}{!}{
\begin{tabular}{c c} % @{\hskip 1em} c}

\AxiomC{$\R, \unda \in D_{w}, w: A(\unda/x), \Gamma \Rightarrow \Delta$}
\RightLabel{$\existsl^{\dag_{3}}$}
\UnaryInfC{$\R, w : \exists x A, \Gamma \Rightarrow \Delta$}
\DisplayProof

&

\AxiomC{$\R, w \leq v, \unda \in D_{v}, v : A(\unda/x), w : \forall x A, \Gamma \Rightarrow \Delta$}
\RightLabel{$\alll$}
\UnaryInfC{$\R, w \leq v, \unda \in D_{v}, w : \forall x A, \Gamma \Rightarrow \Delta$}
\DisplayProof

\end{tabular}
}
\end{center}

\hrule
\caption{The logic ****. The side condition $\dag_{1}$ states that the variable $v$ does not occur in the conclusion, $\dag_{2}$ states that neither $\unda$ nor $v$ occur in the conclusion, and $\dag_{3}$ states that $\unda$ does not occur in the conclusion. Labels and parameters restricted from occurring in the conclusion of an inference are called \emph{eigenvariables}.\protect\footnotemark}
\label{fig:base-calc-lab}
\end{figure}

\footnotetext{Note that $\id$ is an instance of $\idfo$; the same holds in the nested setting.}


{\color{blue} Explain how we extend with properties corresponding to H and HD. Also we use RPi in same way. (2) Explain that most are rule schemes as properties are formula schemes. (3) discuss reflexive case and when antecedent of horn prop is identity. Should include this in logic section as well
}

\begin{figure}
\noindent\hrule

\begin{center}
\begin{tabular}{c c c}
\AxiomC{}
\RightLabel{$\ihd$}
\UnaryInfC{$\R, x :\bot, \Gamma \Rightarrow \Delta$}
\DisplayProof

&

\AxiomC{}
\RightLabel{$\nd$}
\UnaryInfC{$\R, \Gamma \Rightarrow x : \top, \Delta$}
\DisplayProof

&

\AxiomC{$\R, x \leq y, \Gamma \Rightarrow \Delta$}
\RightLabel{$\cd$}
\UnaryInfC{$\R, \Gamma \Rightarrow \Delta$}
\DisplayProof
\end{tabular}
\end{center}



\hrule
\caption{$\dag$ means ****}
\label{fig:extra-rules-lab}
\end{figure}

We define a \emph{label substitution} $(w/v)$ on a labelled sequent in the usual way as the replacement of all labels $v$ occurring in the sequent with the label $w$. Similarly, we define a \emph{parameter substitution} $(a/b)$ on a labelled sequent as the replacement of all parameters $b$ occurring in the sequent with the parameter $a$.


\begin{theorem}
\label{thm:labelled-properties} The calculus ??? have the following properties:
\begin{itemize}

\item[$(i)$] 

\begin{itemize}

\item[(c)] For all $A \in \langsbifo$, $\vdash_{\lcalcsbifo} \R,w \leq v, \vec{\unda} \in D_{w}, w : A(\vec{\unda}), \Gamma \Rightarrow v : A(\vec{\unda}), \Delta$; 

\item[(d)] For all $A \in \langsbifo$, $\vdash_{\lcalcsbifo} \R, \vec{\unda} \in D_{w}, w:A(\vec{\unda}),\Gamma \Rightarrow \Delta, w :A(\vec{\unda})$;

\end{itemize}

\item[$(ii)$] The $(lsub)$ and $(psub)$ rules are height-preserving $($i.e. `hp-'$)$ admissible;
\begin{center}
\begin{tabular}{c @{\hskip 1em} c}
\AxiomC{$\R,\Gamma \Rightarrow \Delta$}
\RightLabel{$(lsub)$}
\UnaryInfC{$\R(w/v),\Gamma(w/v) \Rightarrow \Delta(w/v)$}
\DisplayProof

&

\AxiomC{$\R,\Gamma \Rightarrow \Delta$}
\RightLabel{$(psub)$}
\UnaryInfC{$\R(a/b),\Gamma(a/b) \Rightarrow \Delta(a/b)$}
\DisplayProof
\end{tabular}
\end{center}

%\item[$(iii)$] The parameter substitution rule (below) is hp-admissible;
%\begin{center}
%\AxiomC{$\R,\Gamma \Rightarrow \Delta$}
%\RightLabel{$(psub)$}
%\UnaryInfC{$\R[a/b],\Gamma[a/b] \Rightarrow \Delta[a/b]$}
%\DisplayProof
%\end{center}

\item[$(iii)$] All rules are hp-invertible;

\item[$(iv)$] The $\wk$ and $\{(ctr_{R}),(ctr_{F_{l}}),(ctr_{F_{r}})\}$ rules (below) are hp-admissible;

\begin{center}
\begin{tabular}{c @{\hskip 2em} c} % @{\hskip 1em} c}
\AxiomC{$\R,\Gamma \Rightarrow \Delta$}
\RightLabel{$(wk)$}
\UnaryInfC{$\R',\R,\Gamma',\Gamma \Rightarrow \Delta',\Delta$}
\DisplayProof

&

\AxiomC{$\R,\R',\R',\Gamma \Rightarrow \Delta$}
\RightLabel{$(ctr_{R})$}
\UnaryInfC{$\R,\R',\Gamma \Rightarrow \Delta$}
\DisplayProof

\end{tabular}
\end{center}
\begin{center}
\begin{tabular}{c @{\hskip 2em} c} % @{\hskip 1em} c}

\AxiomC{$\R,\Gamma',\Gamma',\Gamma \Rightarrow \Delta$}
\RightLabel{$(ctr_{F_{l}})$}
\UnaryInfC{$\R,\Gamma',\Gamma \Rightarrow \Delta$}
\DisplayProof

&

\AxiomC{$\R,\Gamma \Rightarrow \Delta, \Delta', \Delta'$}
\RightLabel{$(ctr_{F_{r}})$}
\UnaryInfC{$\R,\Gamma \Rightarrow \Delta, \Delta'$}
\DisplayProof
\end{tabular}
\end{center}

\item[$(v)$] The $\cut$ rule (below) is admissible;

\begin{center}
\begin{tabular}{c}
\AxiomC{$\R,\Gamma \Rightarrow \Delta, w :A$}
\AxiomC{$\R,w :A,\Gamma \Rightarrow \Delta$}
\RightLabel{$\cut$}
\BinaryInfC{$\R,\Gamma \Rightarrow \Delta$}
\DisplayProof
\end{tabular}
\end{center}

\item[$(vi)$] $\lcalcsbifo$ is sound and complete for $\sbifo{\psetsbifo}$.

\end{itemize}
\end{theorem}

\begin{proof} The proofs of properties (i)--(vi) can be found in Appendix~\ref{???}.
\end{proof}







==> Old Files/SEC-LabCalc-SubBiInt.tex <==


{\color{blue} Must consider closure condition. (2) DONT FORGET NED RULE}

We define our labelled sequents to be syntactic objects of the form $L_{1} \Rightarrow L_{2}$, where $L_{1}$ and $L_{2}$ are formulae defined via the BNF grammar below:
\begin{center}
\begin{tabular}{c @{\hskip 2em} c}
$L_{1} ::= w : A \ | \ w \leq u \ | \ L_{1},L_{1}$

&

$L_{2} ::= w : A \ | \ L_{2},L_{2}$
\end{tabular}
\end{center}
where $A$ is in the language $\langsbi$ and $w$ is among a denumerable set of labels $\{w, u, v, \ldots \}$. We refer to formulae of the forms $w \leq u$ as \emph{relational atoms} and refer to formulae of the form $w : A$ as \emph{labelled formulae}. Due to the two types of formulae occurring in a labelled sequent, we often use $\R$ to denote relational atoms, and $\Gamma$ and $\Delta$ to denote labelled formulae, thus distinguishing between the two. Labelled sequents are therefore written in a general form as $\R, \Gamma \Rightarrow \Delta$. Moreover, we take the comma operator to be commutative and associative; for example, we identify the labelled sequent $w \leq u, w : A, w \leq v \sar u :B, v : C$ with $w \leq v, w \leq u, w : A \sar v : C, u :B$. This interpretation of comma lets us view $\R, \Gamma$ and $\Delta$ as multisets. Also, we allow for empty antecedents and succedents in both our labelled and nested sequents.

\begin{figure}
\noindent\hrule

\begin{center}
\begin{tabular}{c @{\hskip 1em} c} % @{\hskip 1em} c}

\AxiomC{}
\RightLabel{$\id$}
\UnaryInfC{$\R,x :p,\Gamma \Rightarrow \Delta, x :p$}
\DisplayProof

&

\AxiomC{$\R, w \leq v, v :A, \Gamma \Rightarrow \Delta, v :B$}
\RightLabel{$\impr^{\dag}$}
\UnaryInfC{$\R, \Gamma \Rightarrow \Delta, w :A \imp B$}
\DisplayProof

\end{tabular}
\end{center}

\begin{center}
\begin{tabular}{c @{\hskip 1em} c @{\hskip 1em} c}

\AxiomC{$\R,w :A, w :B, \Gamma \Rightarrow \Delta$}
\RightLabel{$\conl$}
\UnaryInfC{$\R, w :A \wedge B, \Gamma \Rightarrow \Delta$}
\DisplayProof

&

\AxiomC{$\R, \Gamma \Rightarrow \Delta, w :A$}
\AxiomC{$\R, \Gamma \Rightarrow \Delta, w :B$}
\RightLabel{$\conr$}
\BinaryInfC{$\R, \Gamma \Rightarrow \Delta, w :A \wedge B$}
\DisplayProof

\end{tabular}
\end{center}

\begin{center}
\begin{tabular}{c @{\hskip 1em} c @{\hskip 1em} c}

\AxiomC{$\R, w :A, \Gamma \Rightarrow \Delta$}
\AxiomC{$\R, w :B, \Gamma \Rightarrow \Delta$}
\RightLabel{$\disl$}
\BinaryInfC{$\R, w :A \vee B, \Gamma \Rightarrow \Delta$}
\DisplayProof

&

\AxiomC{$\R, \Gamma \Rightarrow \Delta, w :A, w :B$}
\RightLabel{$\disr$}
\UnaryInfC{$\R, \Gamma \Rightarrow \Delta, w :A \vee B$}
\DisplayProof

\end{tabular}
\end{center}

%\begin{center}
%\begin{tabular}{c}

%\AxiomC{$\R, w \leq v, v :A, \Gamma \Rightarrow \Delta, v :B$}
%\RightLabel{$\imprr^{\dag_{1}}$}
%\UnaryInfC{$\R, \Gamma \Rightarrow \Delta, w :A \imp B$}
%\DisplayProof

%\end{tabular}
%\end{center}

\begin{center}
\begin{tabular}{c}
\AxiomC{$\R,w \leq v, w :A \imp B, \Gamma \Rightarrow \Delta, v :A$}
\AxiomC{$\R,w \leq v, w :A \imp B, v :B, \Gamma \Rightarrow \Delta$}
\RightLabel{$\impl$}
\BinaryInfC{$\R,w \leq v, w :A \imp B, \Gamma \Rightarrow \Delta$}
\DisplayProof 
\end{tabular}
\end{center}

\begin{center}
\begin{tabular}{c}
\AxiomC{$\R,v \leq w, \Gamma \Rightarrow v : A, \Delta$}
\AxiomC{$\R,v \leq w, v : B, \Gamma \Rightarrow w : A \exc B, \Delta$}
\RightLabel{$\excr$}
\BinaryInfC{$\R, v \leq w, \Gamma \Rightarrow w : A \exc B, \Delta$}
\DisplayProof 
\end{tabular}
\end{center}


\begin{center}
\begin{tabular}{c c}

\AxiomC{$\R, v \leq w, v :A, \Gamma \Rightarrow \Delta, v :B$}
\RightLabel{$\excl^{\dag}$}
\UnaryInfC{$\R, \Gamma, w :A \exc B \Rightarrow \Delta$}
\DisplayProof

\end{tabular}
\end{center}


\hrule
\caption{The base labelled calculus $\lcalcsbi$ for the logic $\sbi$. The side condition $\dag$ states that the variable $v$ is an \emph{eigenvariable}, i.e. it does not occur in the conclusion.}
\label{fig:base-calc-lab}
\end{figure}


{\color{blue} Explain how we extend with properties corresponding to H and HD. Also we use RPi in same way. (2) Explain that most are rule schemes as properties are formula schemes. (3) discuss reflexive case and when antecedent of horn prop is identity. Should include this in logic section as well
}

\begin{figure}
\noindent\hrule

\begin{center}
\begin{tabular}{c c c}
\AxiomC{}
\RightLabel{$\botl$}
\UnaryInfC{$\R, x :\bot, \Gamma \Rightarrow \Delta$}
\DisplayProof

&

\AxiomC{}
\RightLabel{$\topr$}
\UnaryInfC{$\R, \Gamma \Rightarrow x : \top, \Delta$}
\DisplayProof

&

\AxiomC{$\R, x \leq x, \Gamma \Rightarrow \Delta$}
\RightLabel{$\refl$}
\UnaryInfC{$\R, \Gamma \Rightarrow \Delta$}
\DisplayProof
\end{tabular}
\end{center}

\begin{center}
\begin{tabular}{c @{\hskip 1em} c}

\AxiomC{$\R, x \leq y, \Gamma \Rightarrow \Delta$}
\RightLabel{$\trans$}
\UnaryInfC{$\R, x \leq y, \Gamma \Rightarrow \Delta$}
\DisplayProof

&

\AxiomC{ }
\RightLabel{$\monid$}
\UnaryInfC{$\R, x \leq y, \Gamma, x : p \Rightarrow y : p, \Delta$}
\DisplayProof

\end{tabular}
\end{center}

\hrule
\caption{$\dag$ means ****}
\label{fig:extra-rules-lab}
\end{figure}

We define a \emph{label substitution} $(w/v)$ on a labelled sequent in the usual way as the replacement of all labels $v$ occurring in the sequent with the label $w$. Similarly, we define a \emph{parameter substitution} $(a/b)$ on a labelled sequent as the replacement of all parameters $b$ occurring in the sequent with the parameter $a$.


\begin{theorem}
\label{thm:lcalcsbi-properties} The calculus $\lcalcsbi$ has the following properties:
\begin{itemize}

\item[$(i)$] 

\begin{itemize}

\item[(a)] For all $A \in \langsbi$, $ \vdash_{\lcalcsbi} \R,w \leq v, w : A, \Gamma \Rightarrow v : A, \Delta$;

\item[(b)] For all $A \in \langsbi$, $ \vdash_{\lcalcsbi} \R,w:A,\Gamma \Rightarrow \Delta, w :A$; 

\end{itemize}

\item[$(ii)$] The $(lsub)$ and $(psub)$ rules are height-preserving $($i.e. `hp-'$)$ admissible;
\begin{center}
\begin{tabular}{c @{\hskip 1em} c}
\AxiomC{$\R,\Gamma \Rightarrow \Delta$}
\RightLabel{$(lsub)$}
\UnaryInfC{$\R(w/v),\Gamma(w/v) \Rightarrow \Delta(w/v)$}
\DisplayProof

&

\AxiomC{$\R,\Gamma \Rightarrow \Delta$}
\RightLabel{$(psub)$}
\UnaryInfC{$\R(a/b),\Gamma(a/b) \Rightarrow \Delta(a/b)$}
\DisplayProof
\end{tabular}
\end{center}

%\item[$(iii)$] The parameter substitution rule (below) is hp-admissible;
%\begin{center}
%\AxiomC{$\R,\Gamma \Rightarrow \Delta$}
%\RightLabel{$(psub)$}
%\UnaryInfC{$\R[a/b],\Gamma[a/b] \Rightarrow \Delta[a/b]$}
%\DisplayProof
%\end{center}

\item[$(iii)$] All rules are hp-invertible;

\item[$(iv)$] The $\wk$ and $\{(ctr_{R}),(ctr_{F_{l}}),(ctr_{F_{r}})\}$ rules (below) are hp-admissible;

\begin{center}
\begin{tabular}{c @{\hskip 2em} c} % @{\hskip 1em} c}
\AxiomC{$\R,\Gamma \Rightarrow \Delta$}
\RightLabel{$(wk)$}
\UnaryInfC{$\R',\R,\Gamma',\Gamma \Rightarrow \Delta',\Delta$}
\DisplayProof

&

\AxiomC{$\R,\R',\R',\Gamma \Rightarrow \Delta$}
\RightLabel{$(ctr_{R})$}
\UnaryInfC{$\R,\R',\Gamma \Rightarrow \Delta$}
\DisplayProof

\end{tabular}
\end{center}
\begin{center}
\begin{tabular}{c @{\hskip 2em} c} % @{\hskip 1em} c}

\AxiomC{$\R,\Gamma',\Gamma',\Gamma \Rightarrow \Delta$}
\RightLabel{$(ctr_{F_{l}})$}
\UnaryInfC{$\R,\Gamma',\Gamma \Rightarrow \Delta$}
\DisplayProof

&

\AxiomC{$\R,\Gamma \Rightarrow \Delta, \Delta', \Delta'$}
\RightLabel{$(ctr_{F_{r}})$}
\UnaryInfC{$\R,\Gamma \Rightarrow \Delta, \Delta'$}
\DisplayProof
\end{tabular}
\end{center}

\item[$(v)$] The $\cut$ rule (below) is admissible;

\begin{center}
\begin{tabular}{c}
\AxiomC{$\R,\Gamma \Rightarrow \Delta, w :A$}
\AxiomC{$\R,w :A,\Gamma \Rightarrow \Delta$}
\RightLabel{$\cut$}
\BinaryInfC{$\R,\Gamma \Rightarrow \Delta$}
\DisplayProof
\end{tabular}
\end{center}

\item[$(vi)$] $\lcalcsbi$ is sound and complete for $\sbi{\psetsbi}$.

\end{itemize}
\end{theorem}

\begin{proof} The proofs of properties (i)--(vi) can be found in Appendix~\ref{???}.
\end{proof}









==> Old Files/SEC-Prelim-SubBiInt-FO.tex <==


The language $\langsbifo$ for our first-order logics is defined via the BNF grammar below:
$$
A ::= p(x_{1}, \ldots, x_{n}) \ | \ \bot \ | \ \top \ | \ (A \vee A) \ | \ (A \land A) \ | \ (A \imp A) \ | \ (A \exc A) \ | \ (\forall x) A \ | \ (\exists x) A
$$
where $p$ is among a denumerable set of $n$-ary \emph{predicate symbols} $\pred = \{p, q, r, \ldots\}$ and $x_{1}, \ldots, x_{n}, x$ are \emph{variables} (with $n \in \mathbb{N}$). We refer to formulae of the form $p(x_{1}, \ldots, x_{n})$ as \emph{atomic formulae} when $n > 0$, and refer to formulae of the form $p$ as \emph{propositional variables} when $n=0$ (i.e., a $0$-ary predicate $p$ is a propositional variable).



\begin{definition}[$\sbifo$-Frames, $\sbifo$-Models~\cite{GabSheSkv09}]\label{def:FO-frame-model} We define a \emph{$\sbifo$-frame} to be a tuple $F = (W,\leq,D)$ such that:
\begin{itemize}

\item[$\blacktriangleright$] $W$ is a non-empty set of worlds $w, u, v, \ldots$ called the \emph{domain};

\item[$\blacktriangleright$] $\leq \ \subseteq W \times W$ is a binary relation on $W$;

\item[$\blacktriangleright$] $D$ is a \emph{domain function} mapping world $w \in W$ to non-empty sets $D_{w}$ of \emph{objects} $\{a, b, c, \dots\}$.
\end{itemize}

A \emph{$\sbifo$-model} $M$ is an ordered pair $(F,V)$ where $F$ is a $\sbifo$-frame and $V$ is a \emph{valuation function} such that $V(p,w) \subseteq (D_{w})^{n}$. We uphold the convention in~\cite{GabSheSkv09} and assume that for each world $w \in W$, $(D_{w})^{0} = \{w\}$, so $V(p,w) = \{w\}$ or $V(p,w) = \emptyset$, for a propositional variable $p$ (which includes $\top$ and $\bot$).
%\begin{itemize}
%\item If $p \in \pred$ with $n > 0$, then $V(p,w) \subseteq (D_{w})^{n}$ for all $w \in W$;
%\item If $p$ is a propositional variable, $\top$, or $\bot$, then $V(p) \in 2^{W}$.
%\end{itemize}
%We uphold the convention in~\cite{GabSheSkv09} and assume that for each world $w \in W$, $(D_{w})^{0} = \{w\}$, so $V(p,w) = \{w\}$ or $V(p,w) = \emptyset$, for a propositional variable $p$.
\end{definition}


%Page. 102 of Gabbay %$D$ be a non-empty set of individuals, called \emph{parameters}, not containing any variables.
\begin{definition}[$D_{w}$-Sentence]\label{def:d-sentence} Let $M = (W, \leq,D,V)$ be a $\sbifo$-model with $w \in W$. We define $\langsbi({D_{w}})$ to be the language $\langsbi$ expanded with parameters $\unda, \undb, \undc, \ldots$ corresponding to the objects in the set $D_{w} = \{a, b, c, \ldots \}$. We define a \emph{$D_{w}$-formula} to be a formula in $\langsbi(D_{w})$, and we define a \emph{$D_{w}$-sentence} to be a $D_{w}$-formula that does not contain any free variables. %Last, we use $a, b, c, \ldots$ to denote parameters in a set $D_{w}$.
\end{definition}

**Define universal closure

%Semantic Clauses found on pp. 208-209 of Gabbay
%~\cite{Cor89-1,Iem05,Kri65,TroDal88}
\begin{definition}[First-Order Semantic Clauses]
\label{def:semantic-clauses} Let $M = (W, \leq,D,V)$ be a $\sbifo{\psetsbi}$-model with $w \in W$. The \emph{satisfaction relation} $M,w \Vdash A$ between $w \in W$ of $M$ and a $D_{w}$-sentence $A$ is inductively defined as follows:

\begin{itemize}

\item[$\blacktriangleright$] If $A$ is a propositional variable $p$, $ \top$, or $\bot$, then $M,w \Vdash A$ iff $w \in V(A)$;

\item[$\blacktriangleright$] If $p$ is an $n$-ary predicate symbol $($with $n > 0)$, then $M,w \Vdash p(\unda_{1}, \cdots, \unda_{n})$ iff $(a_{1}, \cdots, a_{n}) \in V(p,w)$;

%\item $M,w \Vdash A \vee B$ iff $M,w \Vdash A$ or $M,w \Vdash B$;

%\item $M,w \Vdash A \land B$ iff $M,w \Vdash A$ and $M,w \Vdash B$;

%\item $M,w \Vdash A \imp_{i} B$ iff for all $u \in W$, if $w \leq_{i} u$ and $M,u \Vdash A$, then $M,u \Vdash B$;

\item[$\blacktriangleright$] $M,w \Vdash \forall x A(x)$ iff for all $u \in W$ and all $a \in D_{u}$, if $w \leq u$, then $M,u \Vdash A(a)$;

\item[$\blacktriangleright$] $M,w \Vdash \exists x A(x)$ iff there exists an $a \in D_{w}$ such that $M,w \Vdash A(a)$.

\end{itemize}
The clauses for the $\lor$, $\land$, $\imp$, and $\exc$ connectives are the same as in Def.~\ref{def:prop-semantic-clauses}. 
%Global Truth Def. 3.2.19 (p. 210) of Gabbay. Validity is Def. 3.2.21 (p. 211) of Gabbay
We say that a formula $A$ is \emph{globally true on $M$}, written $M \Vdash A$, iff $M,u \Vdash \uc A$ for all worlds $u \in W$ of $M$. A formula $A$ is \emph{$\sbifo{\psetsbi}$-valid}, written $ \Vdash_{\sbifo{\psetsbi}} A$, iff it is globally true on all $\sbifo{\psetsbi}$-models.

\end{definition}



\begin{definition}[Properties $\psetsbifo$]\label{def:fo-properties} Let $M = (W,\leq,D,V)$ be a $\sbifo$-model. A \emph{domain horn property (DHP)} is any property of the following form:
\begin{center}
$\displaystyle{\text{For all $w,u \in W$, if } \ a \in D_{w} \ \text{ and } \ \R_{\Pi}wu \ \text{ then, } \ a \in D_{u}.}$
\end{center}
We use $\psetsbifo$ to denote an arbitrary set of $\psetsbi$ properties and domain horn properties.
\end{definition}




{\color{blue} Give table of first-order logics fitting in above schemes}

==> Old Files/SEC-Prelim-SubBiInt.tex <==


{\color{blue} get rid of universals in front of H properties}

The propositional language $\langsbi$ is defined via the BNF grammar shown below:
$$
A ::= p \ | \ \bot \ | \ \top \ | \ (A \vee A) \ | \ (A \wedge A) \ | \ (A \imp A) \ | \ (A \exc A)
$$
where $p$ is among a denumerable set of \emph{propositional variables} $\prop = \{p, q, r, \ldots\}$. %***(1) Explain top, bottom. (2) Explain implication. (3) Explain excl (various names: excl, subtraction, co-im; we opt for co-imp)

%In the semantics below, we take $\bot$ and $\top$ to be propositional variables as well, and will only interpret them in the usual manner as logical constants 

%We define $\neg A := A \imp \bot$ and $\wneg A := \top \exc A$.

%***Paragraph on weak subint logics and my weak logic: History by Corsi and Restall. History of BiInt. My attempt to provide uniform results and proof-theory by starting with weak base logic

\begin{definition}[$\sbi$-Frame, $\sbi$-Model] An \emph{$\sbi$-frame} is an ordered pair $F = (W, \leq)$ such that:
\begin{itemize}

\item[$\blacktriangleright$] $W$ is a non-empty set of worlds $w, u, v, \ldots$ called the \emph{domain};

\item[$\blacktriangleright$] $\leq \ \subseteq W \times W$ is a binary relation on $W$.
\end{itemize}

An \emph{$\sbi$-model} is an ordered pair $M = (F,V)$ where $F$ is an $\sbi$-frame and $V : \prop \cup \{\top,\bot\} \mapsto 2^{W}$ is a \emph{valuation function} mapping each element of $\prop \cup \{\top,\bot\}$ to a subset of $W$.
\end{definition}

%\cite{GabSheSkv09}
\begin{definition}[Semantic Clauses]
\label{def:sbi-semantic-clauses} Let $M = (W,\leq,V)$ be an $\sbi{\psetsbi}$-model with $w \in W$. The \emph{satisfaction relation} $M,w \Vdash A$ between $w \in W$ of $M$ and a formula $A$ from $\langsbi$ is inductively defined as follows:

\begin{itemize}

\item $M,w \Vdash p$ iff $w \in V(p,w)$;

\item $M,w \Vdash A \vee B$ iff $M,w \Vdash A$ or $M,w \Vdash B$;

\item $M,w \Vdash A \land B$ iff $M,w \Vdash A$ and $M,w \Vdash B$;

\item $M,w \Vdash A \imp B$ iff for all $u \in W$, if $w \leq u$ and $M,u \Vdash A$, then $M,u \Vdash B$;

\item $M,w \Vdash A \exc B$ iff there is an $u \in W$ s.t. $u \leq w$, $M,u \Vdash A$, and $M,u \not\Vdash B$;

\end{itemize}

%Global Truth Def. 3.2.19 (p. 210) of Gabbay. Validity is Def. 3.2.21 (p. 211) of Gabbay

We say that a formula $A$ is \emph{globally true on $M$}, written $M \Vdash A$, iff $M,u \Vdash A$ for all worlds $u \in W$ of $M$. A formula $A$ is \emph{$\sbi{\psetsbi}$-valid}, written $ \Vdash_{\sbi{\psetsbi}} A$, iff it is globally true on all $\sbi{\psetsbi}$-models.

%We say that a set $\Theta$ of formulae \emph{semantically implies} a formula $A$, written $\Theta \Vdash A$, iff for all intuitionistic models $M$ with $w \in W$ of $M$, if $M,w \Vdash B$ for all $B \in \Theta$, then $M,w \Vdash A$.
\end{definition}

The base logic $\sbi$ is defined as the set of all formulae from $\langsbi$ valid on all $\langsbi$-frames (see Def.~\ref{def:prop-semantic-clauses} below). Since part of our aim is to provide a uniform proof-theory for a large class of logics encompassing many well-known propositional and first-order (sub-)intuitionistic logics (potentially with co-implication), we introduce various generalizations of properties often imposed on the models of such logics. These properties include reflexivity, transitivity, truth-persistence, false-persistence, and absurdity, among many others (cf.~\cite{Cor87,IshKash08,Res94}). A collection of commonly studied properties (including the aforementioned ones), their associated logics, and relevant literature is provided in table~\ref{?} below.

Most properties we consider intuitively involve a notion of \emph{reachability}, where, if a certain \emph{path} occurs in a frame with data present at the start of the path, then this implies the existence of some data occurring at the end of the path. For example, truth-persistence---a fundamental property of the relational models employed in intuitionistic logic---states that if $w \in V(p)$ and $w \leq u$, then $u \in V(p)$, i.e., if a propositonal variable $p$ is satisfied at a world $w$ in a model and $w$ sees another world $v$, then $p$ is satisfied at $v$ as well (cf.~\cite{Kri65}). Therefore, we introduce a concise notation to represent a \emph{path} in a model.

\begin{definition}[Path] Let $\sim \ \in \{\leq, \geq\}$. We say that there exists a \emph{path} from $w$ to $u$ iff $w = u$, $w \sim u$, or there exist worlds $v_{i}$ (with $i \in \{1, \ldots, n\}$) such that $w \sim v_{1}, \ldots, v_{n} \sim u$ holds. We use the notation $\R_{\Pi}wu$, $\R_{\Pi'}wu$, $\ldots$ to denote paths from $w$ to $u$.
\end{definition}

***Mention that MHPs capture falsity-persistence as well***

***Given first-order fomrula representation below as well since it is more useful***

\begin{definition}[$\psetsbi$ Properties]\label{def:properties} Let $M = (W,\leq,V)$ be an $\sbi$-model. A \emph{relational horn property (RHP)} is any property of the following form:
\begin{center}
$\displaystyle{\text{For all $w, \ldots, u \in W$, if } \ \R_{\Pi}wu \ \text{ then, } \ w R u.}$
\end{center}
A \emph{monotonic horn property (MHP)} is a property of the following form:
\begin{center}
$\displaystyle{\text{For all $w, \ldots, u \in W$, if } \ w \in V(p) \ \text{ and } \ \R_{\Pi}wu \ \text{ then, } \ u \in V(p).}$
\end{center}
The two \emph{serality properties (D\textsubscript{1} and D\textsubscript{2})} (depending on if $w \sim u$ is $w \leq u$ or $u \leq w$, resp.) are defined as follows:
$$
\text{For all $w \in W$, there exists a $u \in W$ such that } w \sim u.
$$
Last, we introduce the \emph{logical constant properties (LCP)}:
$$
\text{For all $w$, $w \not\in V(\bot)$.} \qquad \text{For all $w$, $w \in V(\top)$.} 
$$
We use $\psetsbi$ to denote an arbitrary set of the above properties.
\end{definition}


%Pg. 140 Domain D_{\Gamma} of theory defined
%Kripke models for FO Intermediate Logics Pg. 205 of Gabbay
%~\cite{Cor89-1,Iem05,TroDal88}
\begin{definition}[$\sbi{\psetsbi}$-Frame, $\sbi{\psetsbi}$-Model]\label{def:LH-frame-model} Let $\psetsbi$ be an arbitrary set of properties. An \emph{$\sbi{\psetsbi}$-frame} is an $\sbi$-frame satisfying each property in $\psetsbi$.\footnote{Note that the only properties that can be imposed on frames are relational horn properties and the seriality properties since monotonic horn properties and logical constant properties incorporate the notion of a valuation.} An \emph{$\sbi{\psetsbi}$-model} is an $\sbi$-model satisfying each property in $\psetsbi$.
\end{definition}





{\color{blue} (0) Mention that semantics is same and define other logics; ACTUALLY, semantics is defined in general above, so mention above that we define in general first (1) Define logic as set of validities (2) Give table of instances of known logics such as dosens, Vissers, biint, Restalls, Corsis}


%By Def.~\ref{def:semantic-clauses} above, the monotonicity condition of Def.~\ref{def:frame-model} can be restated as: for any intuitionistic model $M$ with $w$ and $v$ in the domain $W$ of $M$, if $w \leq v$ and $M,w \Vdash p$, then $M,v \Vdash p$. It is a useful fact that this statement generalizes to arbitrary formulae, and will be leveraged in Section~\ref{section-3} when deriving the nested calculus from the labelled calculus.

%Lem 3.2.16 Gabbay (p. 209)
%\begin{lemma}[General Monotonicity~\cite{GabSheSkv09}]\label{lm:persistency} %~{\cite[Lem.~3.2.16]{GabSheSkv09}}]
%\label{lm:persistency} Let $M$ be a model with domain $W$ and $w,u \in W$. If $w \leq u$ and $M,w \Vdash A$, then $M,u \Vdash A$.
%\end{lemma}







%\resizebox{\columnwidth}{!}{



==> Old Files/body-1.tex <==

\subsection{Propositional Logics}

{\color{blue} get rid of universals in front of H properties}

The propositional language $\lang$ is defined via the BNF grammar shown below:
$$
A ::= p \ | \ \bot \ | \ \top \ | \ (A \vee A) \ | \ (A \wedge A) \ | \ (A \imp A) \ | \ (A \exc A)
$$
where $p$ is among a denumerable set of \emph{propositional variables} $\prop = \{p, q, r, \ldots\}$. %***(1) Explain top, bottom. (2) Explain implication. (3) Explain excl (various names: excl, subtraction, co-im; we opt for co-imp)

%In the semantics below, we take $\bot$ and $\top$ to be propositional variables as well, and will only interpret them in the usual manner as logical constants 

%We define $\neg A := A \imp \bot$ and $\wneg A := \top \exc A$.

%***Paragraph on weak subint logics and my weak logic: History by Corsi and Restall. History of BiInt. My attempt to provide uniform results and proof-theory by starting with weak base logic

\begin{definition}[$\logic$-Frame, $\logic$-Model] An \emph{$\logic$-frame} is an ordered pair $F = (W, \leq)$ such that:
\begin{itemize}

\item[$\blacktriangleright$] $W$ is a non-empty set of worlds $w, u, v, \ldots$ called the \emph{domain};

\item[$\blacktriangleright$] $\leq \ \subseteq W \times W$ is a binary relation on $W$.
\end{itemize}

An \emph{$\logic$-model} is an ordered pair $M = (F,V)$ where $F$ is an $\logic$-frame and $V : \prop \cup \{\top,\bot\} \mapsto 2^{W}$ is a \emph{valuation function} mapping each element of $\prop \cup \{\top,\bot\}$ to a subset of $W$.
\end{definition}

%\cite{GabSheSkv09}
\begin{definition}[Propositional Semantic Clauses]
\label{def:prop-semantic-clauses} Let $M = (W,\leq,V)$ be an $\logic{\hornset}$-model with $w \in W$. The \emph{satisfaction relation} $M,w \Vdash A$ between $w \in W$ of $M$ and a formula $A$ from $\lang$ is inductively defined as follows:

\begin{itemize}

\item $M,w \Vdash p$ iff $w \in V(p,w)$;

\item $M,w \Vdash A \vee B$ iff $M,w \Vdash A$ or $M,w \Vdash B$;

\item $M,w \Vdash A \land B$ iff $M,w \Vdash A$ and $M,w \Vdash B$;

\item $M,w \Vdash A \imp B$ iff for all $u \in W$, if $w \leq u$ and $M,u \Vdash A$, then $M,u \Vdash B$;

\item $M,w \Vdash A \exc B$ iff there is an $u \in W$ s.t. $u \leq w$, $M,u \Vdash A$, and $M,u \not\Vdash B$;

\end{itemize}

%Global Truth Def. 3.2.19 (p. 210) of Gabbay. Validity is Def. 3.2.21 (p. 211) of Gabbay

We say that a formula $A$ is \emph{globally true on $M$}, written $M \Vdash A$, iff $M,u \Vdash A$ for all worlds $u \in W$ of $M$. A formula $A$ is \emph{$\logic{\hornset}$-valid}, written $ \Vdash_{\logic{\hornset}} A$, iff it is globally true on all $\logic{\hornset}$-models.

%We say that a set $\Theta$ of formulae \emph{semantically implies} a formula $A$, written $\Theta \Vdash A$, iff for all intuitionistic models $M$ with $w \in W$ of $M$, if $M,w \Vdash B$ for all $B \in \Theta$, then $M,w \Vdash A$.
\end{definition}

The base logic $\logic$ is defined as the set of all formulae from $\lang$ valid on all $\lang$-frames (see Def.~\ref{def:prop-semantic-clauses} below). Since part of our aim is to provide a uniform proof-theory for a large class of logics encompassing many well-known propositional and first-order (sub-)intuitionistic logics (potentially with co-implication), we introduce various generalizations of properties often imposed on the models of such logics. These properties include reflexivity, transitivity, truth-persistence, false-persistence, and absurdity, among many others (cf.~\cite{Cor87,IshKash08,Res94}). A collection of commonly studied properties (including the aforementioned ones), their associated logics, and relevant literature is provided in table~\ref{?} below.

Most properties we consider intuitively involve a notion of \emph{reachability}, where, if a certain \emph{path} occurs in a frame with data present at the start of the path, then this implies the existence of some data occurring at the end of the path. For example, truth-persistence---a fundamental property of the relational models employed in intuitionistic logic---states that if $w \in V(p)$ and $w \leq u$, then $u \in V(p)$, i.e., if a propositonal variable $p$ is satisfied at a world $w$ in a model and $w$ sees another world $v$, then $p$ is satisfied at $v$ as well (cf.~\cite{Kri65}). Therefore, we introduce a concise notation to represent a \emph{path} in a model.

\begin{definition}[Path] Let $\sim \ \in \{\leq, \geq\}$. We say that there exists a \emph{path} from $w$ to $u$ iff $w = u$, $w \sim u$, or there exist worlds $v_{i}$ (with $i \in \{1, \ldots, n\}$) such that $w \sim v_{1}, \ldots, v_{n} \sim u$ holds. We use the notation $\R_{\Pi}wu$, $\R_{\Pi'}wu$, $\ldots$ to denote paths from $w$ to $u$.
\end{definition}

***Mention that MHPs capture falsity-persistence as well***

***Given first-order fomrula representation below as well since it is more useful***

\begin{definition}[$\hornset$ Properties]\label{def:properties} Let $M = (W,\leq,V)$ be an $\logic$-model. A \emph{relational horn property (RHP)} is any property of the following form:
\begin{center}
$\displaystyle{\text{For all $w, \ldots, u \in W$, if } \ \R_{\Pi}wu \ \text{ then, } \ w R u.}$
\end{center}
A \emph{monotonic horn property (MHP)} is a property of the following form:
\begin{center}
$\displaystyle{\text{For all $w, \ldots, u \in W$, if } \ w \in V(p) \ \text{ and } \ \R_{\Pi}wu \ \text{ then, } \ u \in V(p).}$
\end{center}
The two \emph{serality properties (D\textsubscript{1} and D\textsubscript{2})} (depending on if $w \sim u$ is $w \leq u$ or $u \leq w$, resp.) are defined as follows:
$$
\text{For all $w \in W$, there exists a $u \in W$ such that } w \sim u.
$$
Last, we introduce the \emph{logical constant properties (LCP)}:
$$
\text{For all $w$, $w \not\in V(\bot)$.} \qquad \text{For all $w$, $w \in V(\top)$.} 
$$
We use $\hornset$ to denote an arbitrary set of the above properties.
\end{definition}


%Pg. 140 Domain D_{\Gamma} of theory defined
%Kripke models for FO Intermediate Logics Pg. 205 of Gabbay
%~\cite{Cor89-1,Iem05,TroDal88}
\begin{definition}[$\logic{\hornset}$-Frame, $\logic{\hornset}$-Model]\label{def:LH-frame-model} Let $\hornset$ be an arbitrary set of properties. An \emph{$\logic{\hornset}$-frame} is an $\logic$-frame satisfying each property in $\hornset$.\footnote{Note that the only properties that can be imposed on frames are relational horn properties and the seriality properties since monotonic horn properties and logical constant properties incorporate the notion of a valuation.} An \emph{$\logic{\hornset}$-model} is an $\logic$-model satisfying each property in $\hornset$.
\end{definition}





{\color{blue} (0) Mention that semantics is same and define other logics; ACTUALLY, semantics is defined in general above, so mention above that we define in general first (1) Define logic as set of validities (2) Give table of instances of known logics such as dosens, Vissers, biint, Restalls, Corsis}


%By Def.~\ref{def:semantic-clauses} above, the monotonicity condition of Def.~\ref{def:frame-model} can be restated as: for any intuitionistic model $M$ with $w$ and $v$ in the domain $W$ of $M$, if $w \leq v$ and $M,w \Vdash p$, then $M,v \Vdash p$. It is a useful fact that this statement generalizes to arbitrary formulae, and will be leveraged in Section~\ref{section-3} when deriving the nested calculus from the labelled calculus.

%Lem 3.2.16 Gabbay (p. 209)
%\begin{lemma}[General Monotonicity~\cite{GabSheSkv09}]\label{lm:persistency} %~{\cite[Lem.~3.2.16]{GabSheSkv09}}]
%\label{lm:persistency} Let $M$ be a model with domain $W$ and $w,u \in W$. If $w \leq u$ and $M,w \Vdash A$, then $M,u \Vdash A$.
%\end{lemma}







%\resizebox{\columnwidth}{!}{



\subsection{First-Order Logics}

The language $\langfo$ for our first-order logics is defined via the BNF grammar below:
$$
A ::= p(x_{1}, \ldots, x_{n}) \ | \ \bot \ | \ \top \ | \ (A \vee A) \ | \ (A \land A) \ | \ (A \imp A) \ | \ (A \exc A) \ | \ (\forall x) A \ | \ (\exists x) A
$$
where $p$ is among a denumerable set of $n$-ary \emph{predicate symbols} $\pred = \{p, q, r, \ldots\}$ and $x_{1}, \ldots, x_{n}, x$ are \emph{variables} (with $n \in \mathbb{N}$). We refer to formulae of the form $p(x_{1}, \ldots, x_{n})$ as \emph{atomic formulae} when $n > 0$, and refer to formulae of the form $p$ as \emph{propositional variables} when $n=0$ (i.e., a $0$-ary predicate $p$ is a propositional variable).



\begin{definition}[$\logicfo$-Frames, $\logicfo$-Models~\cite{GabSheSkv09}]\label{def:FO-frame-model} We define a \emph{$\logicfo$-frame} to be a tuple $F = (W,\leq,D)$ such that:
\begin{itemize}

\item[$\blacktriangleright$] $W$ is a non-empty set of worlds $w, u, v, \ldots$ called the \emph{domain};

\item[$\blacktriangleright$] $\leq \ \subseteq W \times W$ is a binary relation on $W$;

\item[$\blacktriangleright$] $D$ is a \emph{domain function} mapping world $w \in W$ to non-empty sets $D_{w}$ of \emph{objects} $\{a, b, c, \dots\}$.
\end{itemize}

A \emph{$\logicfo$-model} $M$ is an ordered pair $(F,V)$ where $F$ is a $\logicfo$-frame and $V$ is a \emph{valuation function} such that $V(p,w) \subseteq (D_{w})^{n}$. We uphold the convention in~\cite{GabSheSkv09} and assume that for each world $w \in W$, $(D_{w})^{0} = \{w\}$, so $V(p,w) = \{w\}$ or $V(p,w) = \emptyset$, for a propositional variable $p$ (which includes $\top$ and $\bot$).
%\begin{itemize}
%\item If $p \in \pred$ with $n > 0$, then $V(p,w) \subseteq (D_{w})^{n}$ for all $w \in W$;
%\item If $p$ is a propositional variable, $\top$, or $\bot$, then $V(p) \in 2^{W}$.
%\end{itemize}
%We uphold the convention in~\cite{GabSheSkv09} and assume that for each world $w \in W$, $(D_{w})^{0} = \{w\}$, so $V(p,w) = \{w\}$ or $V(p,w) = \emptyset$, for a propositional variable $p$.
\end{definition}


%Page. 102 of Gabbay %$D$ be a non-empty set of individuals, called \emph{parameters}, not containing any variables.
\begin{definition}[$D_{w}$-Sentence]\label{def:d-sentence} Let $M = (W, \leq,D,V)$ be a $\logicfo$-model with $w \in W$. We define $\langfo({D_{w}})$ to be the language $\langfo$ expanded with parameters $\unda, \undb, \undc, \ldots$ corresponding to the objects in the set $D_{w} = \{a, b, c, \ldots \}$. We define a \emph{$D_{w}$-formula} to be a formula in $\langfo(D_{w})$, and we define a \emph{$D_{w}$-sentence} to be a $D_{w}$-formula that does not contain any free variables. %Last, we use $a, b, c, \ldots$ to denote parameters in a set $D_{w}$.
\end{definition}

**Define universal closure

%Semantic Clauses found on pp. 208-209 of Gabbay
%~\cite{Cor89-1,Iem05,Kri65,TroDal88}
\begin{definition}[First-Order Semantic Clauses]
\label{def:semantic-clauses} Let $M = (W, \leq,D,V)$ be a $\logicfo{\hornset}$-model with $w \in W$. The \emph{satisfaction relation} $M,w \Vdash A$ between $w \in W$ of $M$ and a $D_{w}$-sentence $A$ is inductively defined as follows:

\begin{itemize}

\item[$\blacktriangleright$] If $A$ is a propositional variable $p$, $ \top$, or $\bot$, then $M,w \Vdash A$ iff $w \in V(A)$;

\item[$\blacktriangleright$] If $p$ is an $n$-ary predicate symbol $($with $n > 0)$, then $M,w \Vdash p(\unda_{1}, \cdots, \unda_{n})$ iff $(a_{1}, \cdots, a_{n}) \in V(p,w)$;

%\item $M,w \Vdash A \vee B$ iff $M,w \Vdash A$ or $M,w \Vdash B$;

%\item $M,w \Vdash A \land B$ iff $M,w \Vdash A$ and $M,w \Vdash B$;

%\item $M,w \Vdash A \imp_{i} B$ iff for all $u \in W$, if $w \leq_{i} u$ and $M,u \Vdash A$, then $M,u \Vdash B$;

\item[$\blacktriangleright$] $M,w \Vdash \forall x A(x)$ iff for all $u \in W$ and all $a \in D_{u}$, if $w \leq u$, then $M,u \Vdash A(a)$;

\item[$\blacktriangleright$] $M,w \Vdash \exists x A(x)$ iff there exists an $a \in D_{w}$ such that $M,w \Vdash A(a)$.

\end{itemize}
The clauses for the $\lor$, $\land$, $\imp$, and $\exc$ connectives are the same as in Def.~\ref{def:prop-semantic-clauses}. 
%Global Truth Def. 3.2.19 (p. 210) of Gabbay. Validity is Def. 3.2.21 (p. 211) of Gabbay
We say that a formula $A$ is \emph{globally true on $M$}, written $M \Vdash A$, iff $M,u \Vdash \uc A$ for all worlds $u \in W$ of $M$. A formula $A$ is \emph{$\logicfo{\hornset}$-valid}, written $ \Vdash_{\logicfo{\hornset}} A$, iff it is globally true on all $\logicfo{\hornset}$-models.

\end{definition}



\begin{definition}[Properties $\hornsetfo$]\label{def:fo-properties} Let $M = (W,\leq,D,V)$ be a $\logicfo$-model. A \emph{domain horn property (DHP)} is any property of the following form:
\begin{center}
$\displaystyle{\text{For all $w,u \in W$, if } \ a \in D_{w} \ \text{ and } \ \R_{\Pi}wu \ \text{ then, } \ a \in D_{u}.}$
\end{center}
We use $\hornsetfo$ to denote an arbitrary set of $\hornset$ properties and domain horn properties.
\end{definition}




{\color{blue} Give table of first-order logics fitting in above schemes}

==> Old Files/internal-external.tex <==



==> Old Files/propositional-int.tex <==


We define \emph{propositional labelled sequents} to be syntactic objects of the form $L_{1} \Rightarrow L_{2}$, where $L_{1}$ and $L_{2}$ are formulae defined via the BNF grammar below top (below bottom, resp.). %Also, we use $\varepsilon$ to represent the empty string, thus allowing empty antecedents or succedents to occur in our labelled sequents.
\begin{center}
\begin{tabular}{c @{\hskip 2em} c}
$L_{1} ::= w : A \ | \ w \leq v \ | \ L_{1},L_{1}$

&

$L_{2} ::= w : A \ | \ L_{2},L_{2}$
\end{tabular}
\end{center}

In the propositional case, $A$ is in the language $\mathcal{L}$ and $x$ is among a denumerable set of labels $\{x, y, z, \ldots \}$. We refer to formulae of the form $w \leq u$ as \emph{relational atoms}, and refer to formulae of the form $w : A$ as \emph{labelled formulae}. Due to the two types of formulae occurring in a labelled sequent, we often use $\R$ to denote relational atoms, and $\Gamma$ and $\Delta$ to denote labelled formulae, thus distinguishing between the two. Labelled sequents are therefore written in a general form as $\R, \Gamma \Rightarrow \Delta$. Moreover, we take the comma operator to be commutative and associative; for example, we identify the labelled sequent $w : A, w \leq u, u :B$ with $w \leq u, u :B, w : A$. This interpretation of comma lets us view $\R, \Gamma$ and $\Delta$ as multisets. Also, we allow for empty antecedents and succedents in both our labelled and nested sequents.

The labelled calculus is given in Fig.~\ref{fig:propositional-calculus}.


\begin{figure}
\noindent\hrule

\begin{center}
\begin{tabular}{c @{\hskip 1em} c} % @{\hskip 1em} c}

\AxiomC{}
\RightLabel{$\id$}
\UnaryInfC{$\R,w \leq v,w :p,\Gamma \Rightarrow \Delta, v :p$}
\DisplayProof

&

\AxiomC{$\R, w \leq v, v :A, \Gamma \Rightarrow \Delta, v :B$}
\RightLabel{$\impr^{\dag_{1}}$}
\UnaryInfC{$\R, \Gamma \Rightarrow \Delta, w :A \imp B$}
\DisplayProof

\end{tabular}
\end{center}

\begin{center}
\begin{tabular}{c @{\hskip 1em} c @{\hskip 1em} c}

\AxiomC{$\R,w :A, w :B, \Gamma \Rightarrow \Delta$}
\RightLabel{$\conl$}
\UnaryInfC{$\R, w :A \wedge B, \Gamma \Rightarrow \Delta$}
\DisplayProof

&

\AxiomC{$\R, \Gamma \Rightarrow \Delta, w :A$}
\AxiomC{$\R, \Gamma \Rightarrow \Delta, w :B$}
\RightLabel{$\conr$}
\BinaryInfC{$\R, \Gamma \Rightarrow \Delta, w :A \wedge B$}
\DisplayProof

\end{tabular}
\end{center}

\begin{center}
\begin{tabular}{c @{\hskip 1em} c @{\hskip 1em} c}

\AxiomC{$\R, w :A, \Gamma \Rightarrow \Delta$}
\AxiomC{$\R, w :B, \Gamma \Rightarrow \Delta$}
\RightLabel{$\disl$}
\BinaryInfC{$\R, w :A \vee B, \Gamma \Rightarrow \Delta$}
\DisplayProof

&

\AxiomC{$\R, \Gamma \Rightarrow \Delta, w :A, w :B$}
\RightLabel{$\disr$}
\UnaryInfC{$\R, \Gamma \Rightarrow \Delta, w :A \vee B$}
\DisplayProof

\end{tabular}
\end{center}

%\begin{center}
%\begin{tabular}{c}

%\AxiomC{$\R, w \leq v, v :A, \Gamma \Rightarrow \Delta, v :B$}
%\RightLabel{$\imprr^{\dag_{1}}$}
%\UnaryInfC{$\R, \Gamma \Rightarrow \Delta, w :A \imp B$}
%\DisplayProof

%\end{tabular}
%\end{center}

\begin{center}
\begin{tabular}{c}
\AxiomC{$\R,w \leq v, w :A \imp B, \Gamma \Rightarrow \Delta, v :A$}
\AxiomC{$\R,w \leq v, w :A \imp B, v :B, \Gamma \Rightarrow \Delta$}
\RightLabel{$\impl$}
\BinaryInfC{$\R,w \leq v, w :A \imp B, \Gamma \Rightarrow \Delta$}
\DisplayProof 
\end{tabular}
\end{center}

\begin{center}
\begin{tabular}{c @{\hskip 1em} c}

\AxiomC{$\R,w \leq w, \Gamma \Rightarrow \Delta$}
\RightLabel{$\refl$}
\UnaryInfC{$\R,\Gamma \Rightarrow \Delta$}
\DisplayProof

&

\AxiomC{$\R,w \leq v, v \leq u, w \leq u, \Gamma \Rightarrow \Delta$}
\RightLabel{$\trans$}
\UnaryInfC{$\R,w \leq v, v \leq u, \Gamma \Rightarrow \Delta$}
\DisplayProof

\end{tabular}
\end{center}

\begin{center}
\begin{tabular}{c @{\hskip 1em} c}
\AxiomC{}
\RightLabel{$\botr$}
\UnaryInfC{$\R,w :\bot, \Gamma \Rightarrow \Delta$}
\DisplayProof

&


\end{tabular}
\end{center}


\begin{center}
\begin{tabular}{c @{\hskip 1em} c}

\AxiomC{$\R, y \leq x, \Gamma \Rightarrow y : A, \Delta$}
\AxiomC{$\R, y \leq x, \Gamma, y : B \Rightarrow \Delta$}
\RightLabel{$\excr$}
\BinaryInfC{$\R, x \leq y, \Gamma \Rightarrow x : A \exc B, \Delta$}
\DisplayProof

&

\AxiomC{$\R, x \leq y, \Gamma, y : A \Rightarrow y : B, \Delta$}
\RightLabel{$\excl^{\dag}$}
\UnaryInfC{$\R, \Gamma, x : A \exc B \Rightarrow \Delta$}
\DisplayProof

\end{tabular}
\end{center}

\hrule
\caption{The labelled calculus ??? for propositional intuitionistic logic ??? The side condition $\dag_{1}$ states that the variable $v$ does not occur in the conclusion, $\dag_{2}$ states that neither $a$ nor $v$ occur in the conclusion, and $\dag_{3}$ states that $a$ does not occur in the conclusion. Labels and parameters restricted from occurring in the conclusion of an inference are called \emph{eigenvariables}.}
\label{fig:subbitint-lab-calc}
\end{figure}


We define a \emph{label substitution} $[x/y]$ on a labelled sequent in the usual way as the replacement of all labels $y$ occurring in the sequent with the label $x$.


\begin{theorem}
\label{thm:lint-properties} The calculi ??? and $???$ have the following properties:
\begin{itemize}

\item[$(i)$] 

\begin{itemize}

\item[(a)] For all $A \in \mathcal{L}$, $ \vdash_{???} \R,w \leq v, w : A, \Gamma \Rightarrow v : A, \Delta$;

\item[(b)] For all $A \in \mathcal{L}$, $ \vdash_{???} \R,w:A,\Gamma \Rightarrow \Delta, w :A$; 

\end{itemize}

\item[$(ii)$] The $(lsub)$ rules are height-preserving $($i.e. `hp-'$)$ admissible;
\begin{center}
\begin{tabular}{c @{\hskip 1em} c}
\AxiomC{$\R,\Gamma \Rightarrow \Delta$}
\RightLabel{$(lsub)$}
\UnaryInfC{$\R[w/v],\Gamma[w/v] \Rightarrow \Delta[w/v]$}
\DisplayProof


\end{tabular}
\end{center}


\item[$(iii)$] All rules are hp-invertible;

\item[$(iv)$] The $\wk$ and $\{(ctr_{R}),(ctr_{F_{l}}),(ctr_{F_{r}})\}$ rules (below) are hp-admissible;

\begin{center}
\begin{tabular}{c @{\hskip 2em} c} % @{\hskip 1em} c}
\AxiomC{$\R,\Gamma \Rightarrow \Delta$}
\RightLabel{$(wk)$}
\UnaryInfC{$\R',\R,\Gamma',\Gamma \Rightarrow \Delta',\Delta$}
\DisplayProof

&

\AxiomC{$\R,\R',\R',\Gamma \Rightarrow \Delta$}
\RightLabel{$\ctrrel$}
\UnaryInfC{$\R,\R',\Gamma \Rightarrow \Delta$}
\DisplayProof

\end{tabular}
\end{center}
\begin{center}
\begin{tabular}{c @{\hskip 2em} c} % @{\hskip 1em} c}

\AxiomC{$\R,\Gamma',\Gamma',\Gamma \Rightarrow \Delta$}
\RightLabel{$\ctrl$}
\UnaryInfC{$\R,\Gamma',\Gamma \Rightarrow \Delta$}
\DisplayProof

&

\AxiomC{$\R,\Gamma \Rightarrow \Delta, \Delta', \Delta'$}
\RightLabel{$\ctrr$}
\UnaryInfC{$\R,\Gamma \Rightarrow \Delta, \Delta'$}
\DisplayProof
\end{tabular}
\end{center}

\item[$(v)$] The $\cut$ rule (below) is admissible;

\begin{center}
\begin{tabular}{c}
\AxiomC{$\R,\Gamma \Rightarrow \Delta, w :A$}
\AxiomC{$\R,w :A,\Gamma \Rightarrow \Delta$}
\RightLabel{$\cut$}
\BinaryInfC{$\R,\Gamma \Rightarrow \Delta$}
\DisplayProof
\end{tabular}
\end{center}

\item[$(vi)$] $???$ $(???focd)$ is sound and complete for ???.

\end{itemize}
\end{theorem}

\begin{proof} We refer the reader to~\cite{DycNeg12} for proofs of properties (i)--(vi) for $???$; note that hp-admissibility of $(psub)$ is trivial in the propositional setting since formulae do not contain parameters. The proofs of properties (i)--(vi) can be found in the online appended version~\cite{LyonArxiv} for ???.
%\qed
\end{proof}

==> intro.tex <==
%% intro.tex
%% Copyright (C) 2014-2020 by Thomas Auzinger <thomas@auzinger.name>
%
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   http://www.latex-project.org/lppl.txt
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
%
% This work has the LPPL maintenance status `maintained'.
%
% The Current Maintainer of this work is Thomas Auzinger.
%
% This work consists of the files vutinfth.dtx and vutinfth.ins
% and the derived file vutinfth.cls.
% This work also consists of the file intro.tex.


\newacronym{ctan}{CTAN}{Comprehensive TeX Archive Network}
\newacronym{faq}{FAQ}{Frequently Asked Questions}
\newacronym{pdf}{PDF}{Portable Document Format}
\newacronym{svn}{SVN}{Subversion}
\newacronym{wysiwyg}{WYSIWYG}{What You See Is What You Get}

\newglossaryentry{texteditor}
{
  name={editor},
  description={A text editor is a type of program used for editing plain text files.}
}

\chapter{Introduction to \LaTeX}

Since \LaTeX\ is widely used in academia and industry, there exists a plethora of freely accessible introductions to the language.
Reading through the guide at \url{https://en.wikibooks.org/wiki/LaTeX} serves as a comprehensive overview for most of the functionality and is highly recommended before starting with a thesis in \LaTeX.

\section{Installation}

A full \LaTeX\ distribution\index{distribution} consists not only of the binaries that convert the source files to the typeset documents, but also of a wide range of packages and their documentation.
Depending on the operating system, different implementations are available as shown in Table~\ref{tab:distrib}.
\textbf{Due to the large amount of packages that are in everyday use and due to their high interdependence, it is paramount to keep the installed distribution\index{distribution} up to date.}
Otherwise, obscure errors and tedious debugging ensue.

\begin{table}
  \centering
  \begin{tabular}{cccc}
    \toprule
    Distribution & Unix         & Windows      & MacOS        \\
    \midrule
    TeX Live     & \textbf{yes} & yes          & (yes)        \\
    MacTeX       & no           & no           & \textbf{yes} \\
    MikTeX       & (yes)        & \textbf{yes} & yes          \\
    \bottomrule
  \end{tabular}
  \caption{\TeX/\LaTeX\ distributions for different operating systems. Recomended choice in \textbf{bold}.}
  \label{tab:distrib} % \label has to be placed AFTER \caption to produce correct cross-references.
\end{table}

\section{Editors}

A multitude of \TeX\ \glspl{texteditor} are available differing in their editing models, their supported operating systems and their feature sets.
A comprehensive overview of \glspl{texteditor} can be found at the Wikipedia page  \url{https://en.wikipedia.org/wiki/Comparison_of_TeX_editors}.
TeXstudio (\url{http://texstudio.sourceforge.net/}) is recommended.
Most editors support a synchronization of the generated document and the \LaTeX\ source by \verb|Ctrl| clicking either on the source document or the generated document.

\section{Compilation}

Modern editors usually provide the compilation programs to generate \gls{pdf} documents and for most \LaTeX\ source files, this is sufficient.
More advanced \LaTeX\ functionality, such as glossaries and bibliographies, needs additional compilation steps, however.
It is also possible that errors in the compilation process invalidate intermediate files and force subsequent compilation runs to fail.
It is advisable to delete intermediate files (\verb|.aux|, \verb|.bbl|, etc.), if errors occur and persist.
All files that are not generated by the user are automatically regenerated.
To compile the current document, the steps as shown in Table~\ref{tab:compile} have to be taken.


\begin{table}
  \centering
  \begin{tabular}{rl}
    \toprule
    & Description \\
    \midrule
    1 & Scan for refs, toc/lof/lot/loa items and cites \\
    2 & Build the bibliography     \\
    3 & Link refs and build the toc/lof/lot/loa \\
    4 & Link the bibliography \\
    5 & Build the glossary \\
    6 & Build the acronyms \\
    7 & Build the index \\
    8 & Link the glossary, acronyms, and the index \\
    9 & Link the bookmarks \\
    \midrule
    & Command \\
    \midrule
    1 & \verb|pdflatex.exe  example| \\
    2 & \verb|bibtex.exe    example| \\
    3 & \verb|pdflatex.exe  example| \\
    4 & \verb|pdflatex.exe  example| \\
    5 & \verb|makeindex.exe -t example.glg -s example.ist| \\
      & \verb|              -o example.gls example.glo| \\
    6 & \verb|makeindex.exe -t example.alg -s example.ist| \\
      & \verb|              -o example.acr example.acn| \\
    7 & \verb|makeindex.exe -t example.ilg -o example.ind example.idx| \\
    8 & \verb|pdflatex.exe  example| \\
    9 & \verb|pdflatex.exe  example| \\
    \bottomrule
  \end{tabular}
  \caption{Compilation steps for this document. The following abbreviations were used: table of contents (toc), list of figures (lof), list of tables (lot), list of algorithms (loa).}
  \label{tab:compile} % \label has to be placed AFTER \caption to produce correct cross-references.
\end{table}


\section{Basic Functionality}

In this section, various examples are given of the fundamental building blocks used in a thesis.
Many \LaTeX\ commands have a rich set of options that can be supplied as optional arguments.
The documentation of each command should be consulted to get an impression of the full spectrum of its functionality.

\subsection{Floats}

Two main categories of page elements can be differentiated in the usual \LaTeX\ workflow: \textit{(i)} the main stream of text and \textit{(ii)} floating containers that are positioned at convenient positions throughout the document.
In most cases, tables, plots, and images are put into such containers since they are usually positioned at the top or bottom of pages.
These are realized by the two environments \verb|figure| and \verb|table|, which also provide functionality for cross-referencing (see Table~\ref{tab:intro} and Figure~\ref{fig:intro}) and the generation of corresponding entries in the list of figures and the list of tables.
Note that these environments solely act as containers and can be assigned arbitrary content.

\subsection{Tables}

A table in \LaTeX\ is created by using a \verb|tabular| environment or any of its extensions, e.g., \verb|tabularx|.
The commands \verb|\multirow| and \verb|\multicolumn| allow table elements to span multiple rows and columns.

\begin{table}[h] % placement specifier
  \centering
  \begin{tabular}{lll}
    \toprule
    \multicolumn{2}{c}{Position} \\
    \cmidrule{1-2} % partial horizontal rule
    Group & Abbrev & Name \\
    \midrule
    Goalkeeper & GK & Paul Robinson \\
    \midrule
    \multirow{4}{*}{Defenders} & LB & Lucus Radebe \\
                               & DC & Michael Duburry \\
                               & DC & Dominic Matteo \\
                               & RB & Didier Domi \\
    \midrule
    \multirow{3}{*}{Midfielders} & MC & David Batty \\
                                 & MC & Eirik Bakke \\
                                 & MC & Jody Morris \\
    \midrule
    Forward & FW & Jamie McMaster \\
    \midrule
    \multirow{2}{*}{Strikers} & ST & Alan Smith \\
                              & ST & Mark Viduka \\
    \bottomrule
  \end{tabular}
  \caption{Adapted example from the \LaTeX guide at \url{https://en.wikibooks.org/wiki/LaTeX/Tables}. This example uses rules specific to the \texttt{booktabs} package and employs the multi-row functionality of the \texttt{multirow} package.}
  \label{tab:intro} % \label has to be placed AFTER \caption to produce correct cross-references.
\end{table}

\subsection{Images}

An image is added to a document via the \verb|\includegraphics| command as shown in Figure~\ref{fig:intro}.
The \verb|\subcaption| command can be used to reference subfigures, such as Figure~\ref{fig:intro:full width} and~\ref{fig:intro:half width}.

\begin{figure}[h]
  \centering
  \begin{subfigure}[b]{0.45\columnwidth}
    \centering
    \includegraphics[width=\textwidth]{Logo-schwarz.pdf}
    \subcaption{The header logo at text width.}
    \label{fig:intro:full width}
  \end{subfigure}
  \begin{subfigure}[b]{0.45\columnwidth}
    \centering
    \includegraphics[width=0.5\textwidth]{Logo-schwarz.pdf}
    \subcaption{The header logo at half the text width.}
    \label{fig:intro:half width}
  \end{subfigure}
  \caption[Optional caption for the figure list (often used to abbreviate long captions)]{The header logo at different sizes.} % Remove the [...] argument if the original caption should be used in the figure list.
  \label{fig:intro} % \label has to be placed AFTER \caption (or \subcaption) to produce correct cross-references.
\end{figure}

\subsection{Mathematical Expressions}

One of the original motivation to create the \TeX\ system was the need for mathematical typesetting.
To this day, \LaTeX\ is the preferred system to write math-heavy documents and a wide variety of functions aids the author in this task.
A mathematical expression can be inserted inline as $\sum_{n=1}^{\infty} \frac{1}{n^2} = \frac{\pi^2}{6}$ outside of the text stream as \[ \sum_{n=1}^{\infty} \frac{1}{n^2} = \frac{\pi^2}{6} \] or as numbered equation with
\begin{equation}
\sum_{n=1}^{\infty} \frac{1}{n^2} = \frac{\pi^2}{6}.
\end{equation}

\subsection{Pseudo Code}

The presentation of algorithms can be achieved with various packages; the most popular are \verb|algorithmic|, \verb|algorithm2e|, \verb|algorithmicx|, or \verb|algpseudocode|.
An overview is given at \url{https://tex.stackexchange.com/questions/229355}.
An example of the use of the \verb|alogrithm2e| package is given with Algorithm~\ref{alg:gauss-seidel}.

\begin{algorithm}
  \SetKw{BreakFor}{break for}
  \KwIn{A scalar~$\epsilon$, a matrix $\mathbf{A} = (a_{ij})$, a vector $\vec{b}$, and an initial vector $\vec{x}^{(0)}$}
  \KwOut{$\vec{x}^{(n)}$ with $\mathbf{A} \vec{x}^{(n)} \approx \vec{b}$}
  \For{$k\leftarrow 1$ \KwTo maximum iterations}
  {
     \For{$i\leftarrow 1$ \KwTo $n$}
     {
        $x_i^{(k)} = \frac{1}{a_{ii}} \left(b_i-\sum_{j<i} a_{ij} x_j^{(k)} - \sum_{j>i} a_{ij} x_j^{(k-1)} \right)$\;
     }
     \If{$\lvert\vec{x}^{(k)}-\vec{x}^{(k-1)}\rvert < \epsilon$}
     {\BreakFor\;}
  }
  \Return{$\vec{x}^{(k)}$\;}
  \caption{Gauss-Seidel}
  \label{alg:gauss-seidel} % \label has to be placed AFTER \caption to produce correct cross-references.
\end{algorithm}

\section{Bibliography}

The referencing of prior work is a fundamental requirement of academic writing and well supported by \LaTeX.
The \textsc{Bib}\TeX\ reference management software is the most commonly used system for this purpose.
Using the \verb|\cite| command, it is possible to reference entries in a \verb|.bib| file out of the text stream, e.g., as~\cite{Turing1936}.
The generation of the formatted bibliography needs a separate execution of \verb|bibtex.exe| (see Table~\ref{tab:compile}).

\section{Table of Contents}

The table of contents is automatically built by successive runs of the compilation, e.g., of \verb|pdflatex.exe|.
The command \verb|\setsecnumdepth| allows the specification of the depth of the table of contents and additional entries can be added to the table of contents using \verb|\addcontentsline|.
The starred versions of the sectioning commands, i.e., \verb|\chapter*|, \verb|\section*|, etc., remove the corresponding entry from the table of contents.

\section{Acronyms / Glossary / Index}

The list of acronyms, the glossary, and the index need to be built with a separate execution of \verb|makeindex| (see Table~\ref{tab:compile}).
Acronyms have to be specified with \verb|\newacronym| while glossary entries use \verb|\newglossaryentry|.
Both are then used in the document content with one of the variants of \verb|\gls|, such as \verb|\Gls|, \verb|\glspl|, or \verb|\Glspl|.
Index items are simply generated by placing \verb|\index|\marg{entry} next to all the words that correspond to the index entry \meta{entry}.
Note that many enhancements exist for these functionalities and the documentation of the \verb|makeindex| and the \verb|glossaries| packages should be consulted.

\section{Tips}

Since \TeX\ and its successors do not employ a \gls{wysiwyg} editing scheme, several guidelines improve the readability of the source content:
\begin{itemize}
\item Each sentence in the source text should start with a new line.
      This helps not only the user navigation through the text, but also enables revision control systems (e.g. \gls{svn}, Git) to show the exact changes authored by different users.
      Paragraphs are separated by one (or more) empty lines.
\item Environments, which are defined by a matching pair of \verb|\begin{name}| and \verb|\end{name}|, can be indented by whitespace to show their hierarchical structure.
\item In most cases, the explicit use of whitespace (e.g. by adding \verb|\hspace{4em}| or \verb|\vspace{1.5cm}|) violates typographic guidelines and rules.
      Explicit formatting should only be employed as a last resort and, most likely, better ways to achieve the desired layout can be found by a quick web search.
\item The use of bold or italic text is generally not supported by typographic considerations and the semantically meaningful \verb|\emph{|\texttt{$\dots$}\verb|}| should be used.
\end{itemize}

The predominant application of the \LaTeX\ system is the generation of \gls{pdf} files via the \textsc{Pdf}\LaTeX\ binaries.
In the current version of \textsc{Pdf}\LaTeX, it is possible that absolute file paths and user account names are embedded in the final \gls{pdf} document.
While this poses only a minor security issue for all documents, it is highly problematic for double blind reviews.
The process shown in Table~\ref{tab:ps2pdf} can be employed to strip all private information from the final \gls{pdf} document.

\begin{table}[h]
  \centering
  \begin{tabular}{rl}
  \toprule
  & Command \\
  \midrule
  1 & Rename the \gls{pdf} document \verb|final.pdf| to \verb|final.ps|. \\
  2 & Execute the following command: \\
    & \verb|ps2pdf -dPDFSETTINGS#/prepress ^| \\
    & \verb| -dCompatibilityLevel#1.4 ^| \\
    & \verb| -dAutoFilterColorImages#false ^| \\
    & \verb| -dAutoFilterGrayImages#false ^| \\
    & \verb| -dColorImageFilter#/FlateEncode ^| \\
    & \verb| -dGrayImageFilter#/FlateEncode ^| \\
    & \verb| -dMonoImageFilter#/FlateEncode ^| \\
    & \verb| -dDownsampleColorImages#false ^| \\
    & \verb| -dDownsampleGrayImages#false ^| \\
    & \verb| final.ps final.pdf| \\
  \bottomrule
  \end{tabular}

  On Unix-based systems, replace \verb|#| with \verb|=| and \verb|^| with \verb|\|.
  \caption{Anonymization of \gls{pdf} documents.}
  \label{tab:ps2pdf}
\end{table}

\section{Resources}

\subsection{Useful Links}

In the following, a listing of useful web resources is given.
\begin{description}
\item[\url{https://en.wikibooks.org/wiki/LaTeX}] An extensive wiki-based guide to \LaTeX.
\item[\url{http://www.tex.ac.uk/faq}] A (huge) set of \gls{faq} about \TeX\ and \LaTeX.
\item[\url{https://tex.stackexchange.com/}] The definitive user forum for non-trivial \LaTeX-related questions and answers.
\end{description}

\subsection[Comprehensive TeX Archive Network]{\gls{ctan}}

The \gls{ctan} is the official repository for all \TeX\ related material.
It can be accessed via \url{https://www.ctan.org/} and hosts (among other things) a huge variety of packages that provide extended functionality for \TeX\ and its successors.
Note that most packages contain \gls{pdf} documentation that can be directly accessed via \gls{ctan}.

In the following, a short, non-exhaustive list of relevant \gls{ctan}-hosted packages is given together with their relative path.
\begin{description}[itemsep=0ex]
\item[\href{https://www.ctan.org/pkg/algorithm2e}{algorithm2e}] Functionality for writing pseudo code.
\item[\href{https://www.ctan.org/pkg/amsmath}{amsmath}] Enhanced functionality for typesetting mathematical expressions.
\item[\href{https://www.ctan.org/pkg/amsfonts}{amssymb}] Provides a multitude of mathematical symbols.
\item[\href{https://www.ctan.org/pkg/booktabs}{booktabs}] Improved typesetting of tables.
\item[\href{https://www.ctan.org/pkg/enumitem}{enumitem}] Control over the layout of lists (\verb|itemize|, \verb|enumerate|, \verb|description|).
\item[\href{https://www.ctan.org/pkg/fontenc}{fontenc}] Determines font encoding of the output.
\item[\href{https://www.ctan.org/pkg/glossaries}{glossaries}] Create glossaries and list of acronyms.
\item[\href{https://www.ctan.org/pkg/graphicx}{graphicx}] Insert images into the document.
\item[\href{https://www.ctan.org/pkg/inputenc}{inputenc}] Determines encoding of the input.
\item[\href{https://www.ctan.org/pkg/l2tabu}{l2tabu}] A description of bad practices when using \LaTeX.
\item[\href{https://www.ctan.org/pkg/mathtools}{mathtools}] Further extension of mathematical typesetting.
\item[\href{https://www.ctan.org/pkg/memoir}{memoir}] The document class on upon which the \verb|vutinfth| document class is based.
\item[\href{https://www.ctan.org/pkg/multirow}{multirow}] Allows table elements to span several rows.
\item[\href{https://www.ctan.org/pkg/pgfplots}{pgfplots}] Function plot drawings.
\item[\href{https://www.ctan.org/pkg/pgf}{pgf/TikZ}] Creating graphics inside \LaTeX\ documents.
\item[\href{https://www.ctan.org/pkg/subcaption}{subcaption}] Allows the use of subfigures and enables their referencing.
\item[\href{https://www.ctan.org/tex-archive/info/symbols/comprehensive/}{symbols/comprehensive}] A listing of around 5000 symbols that can be used with \LaTeX.
\item[\href{https://www.ctan.org/pkg/voss-mathmode}{voss-mathmode}] A comprehensive overview of typesetting mathematics in \LaTeX.
\item[\href{https://www.ctan.org/pkg/xcolor}{xcolor}] Allows the definition and use of colors.
\end{description}

==> notation.tex <==



%Explain Sequent Calculus by Gentzen: Applications and Significance

In his seminal work~\cite{Gen35}, Gentzen proposed the \emph{sequent calculus} framework for classical and intuitionistic logic, and subsequently, proved his celebrated \emph{Hauptsatz} (i.e. cut-elimination theorem), which ultimately provided analytic calculi for the two logics. Gentzen's sequent calculus formalism has become one of the preferred proof-theoretic frameworks for providing analytic calculi, and indeed, many logics of interest have been equipped with such calculi. Nevertheless, one of the alluring features of the formalism---namely, its simplicity---has also proven to be one of the formalism's drawbacks; there remain many logics for which no cut-free, or analytic, sequent calculus (\`a la Gentzen) is known~\cite{GorPosTiu08,Pog08}. In response to this, the sequent calculus formalism has been extended in various ways to include additional structure, allowing for numerous logics to be supplied with cut-free, analytic calculi. Some of the most prominent extensions of Gentzen's formalism include \emph{display calculi}~\cite{Bel82}, \emph{labelled calculi}~\cite{LyoBer19,Vig00}, \emph{hypersequent calculi}~\cite{Pog08}, and \emph{nested calculi}~\cite{Fit14,GorPosTiu08}.


%Explain shortcomings of SC leading to it being generalized to many different formalisms that accommodate many different logics. It was generalized because of shortcomings of SC--more structure added to get cut-elimination, subformula property, and therefore nice consequences such as complexity-optimal decidability, counter-model extraction, interpolation.




%Hypersequents

%2-Sequents, LNS and PLNS

In this paper, we employ the \emph{linear nested sequent} formalism, introduced by Lellmann in~\cite{Lel15}. Linear nested sequents fall within the \emph{nested calculus paradigm}, but where sequents are restricted to linear, instead of treelike, structures. Linear nested sequents are based off of Masini's 2-sequent framework~\cite{Mas92,Mas93} that was used to provide cut-free calculi for the modal logic $\mathsf{KD}$ as well as various other constructive logics. 
The linear nested formalism proves to be highly compatible with the well-known first-order G\"odel logic ??? (i.e. intuitionistic fuzzy logic), due to the fact that ??? can be semantically characterized by \emph{linear} relational frames (see Sect.~\ref{sec:logical-prelims}). The present work provides the linear nested calculus ??? for ???, which enjoys a variety of fruitful properties, such as:\footnote{We refer to~\cite{Wan94} for a detailed discussion of fundamental proof-theoretic properties.}

%Nested Sequents

In 2009, Br\"unnler introduced \emph{nested sequent calculi}~\cite{Bru09} and Poggiolesi introduced \emph{tree hypersequent calculi}~\cite{Pog09Trends} for a set of modal logics. Both formalisms are essentially notational variants of one another and make use of an idea due to Bull~\cite{Bul92} and Kashima~\cite{Kas94} to organize sequents into treelike structures called \emph{nested sequents}. Although nested sequents can be seen as a distinct proof-theoretic formalism, it was shown in 2012~\cite{Fit12} that nested sequent calculi can be viewed as `upside-down' versions of prefixed tableaux, introduced much earlier in 1972~\cite{Fit72}.
In contrast to labelled sequents, nested sequents %prove theorems 
are often given in a language as expressive as the language of the logic; thus, nested calculi have the advantage that they minimize the bureaucracy sufficient to prove theorems. The nested formalism continues to receive much attention, proving itself suitable for constructing analytic calculi~\cite{Bru09}, developing automated reasoning algorithms~\cite{GorPosTiu11}, and verifying interpolation~\cite{LyoTiuGorClo20}, among other applications.

%Display Sequents

%Indexed-Nested Sequents: Fitting, Rosalie

%Labelled Sequents

The labelled approach of constructing calculi may be qualified as \emph{semantic} due to the fact that calculi are obtained through the transformation of semantic clauses and Kripke-frame properties into inference rules for a logic~\cite{DycNeg12,Vig00}. Although the approach has been criticized by some~\cite{Avr96}, it has also proven to be quite successful relative to certain criteria. For example, the labelled formalism is surprisingly modular and allows for the automated construction of analytic calculi for many intermediate and modal logics~\cite{CiaMafSpe13,DycNeg12,Neg16}. Furthermore, calculi constructed in the labelled paradigm often possess fruitful properties (e.g. contraction-admissibility, invertibility of rules, cut-elimination, etc.) that follow from general results~\cite{DycNeg12,Neg16}.

%State that there are other types of calculi: (Prefixed) Tableaux, Calculus of Structures, Tree-Hypersequents, Resolution, Natural Deduction



%Explain theme throughout that structure increases: ioslated points, ..., to arbitrary graphs. Can unify them with underlying graphical structures: graphs with nodes decorated with formulae from context free grammar. Gives substratum to all formalisms and allows for invstigation of those inbetween (e.g., Single-Agent STIT with choice limitation). 



%(Allows general results??? e.g. General Cut-elim. from sufficient conditions). ***Notation matters*** (explain issues with interpolation with HS and how resolved in LNS for Godel-Dummet Logic. IMPORTANT TO MENTION: want to provide general notation that caputures all formalisms; as will be explained, this allows for us to easily transition from high complexity/structural (not in the complexity theoretic sense) systems to less (this will have applications as explained in chapters 5 and 6).



%Notation might be too general, but can simplify without time and gives starting point (e.g. groups, fields, etc.)










\section{A Uniform Notation for Proof Systems}





\begin{definition}[Generalized Sequent] We define a \emph{(generalized) sequent} to be tuple $(V,E,G,D)$, where

\begin{itemize}

\item[$\blacktriangleright$] $V$ is a (possibly infinite) set of vertices;

\item[$\blacktriangleright$] $E = \{E_{n} \ | \ n \in N \subseteq \mathbb{N} \}$ is a set of $n$-ary relations on $V$, i.e. $E_{i} \subseteq \displaystyle{\prod_{1 \leq i \leq n} V}$;

\item[$\blacktriangleright$] $G$ is a context-free grammar (with $\mathcal{L}(G)$ the language generated by the grammar);

\item[$\blacktriangleright$]  $D : V \mapsto \mathcal{L}(G)$ is a decoration function mapping vertices to formulae in the language $\mathcal{L}(G)$ of the grammar $G$.

\end{itemize}

We refer to $(V,E)$ as the \emph{fundamental graph}.

\end{definition}



\begin{definition}[Generalized Sequent Calculus] We define a \emph{Generalized Sequent Calculus} to be an ordered pair $(S,R)$, where

\begin{itemize}

\item[$\blacktriangleright$] $S$ is a set of generalized sequents;

\item[$\blacktriangleright$] $R = \{R_{n} \ | \ \}$ is a set of computable functions $R_{i} : S^{n} \mapsto S$ with $1 \leq i \leq n$. ***Closed under $S$*** (Type of calculus could have $S$ generated by $R$, and some types could not; what does this mean?)

\end{itemize}

\end{definition}

%Explain how rules are typically represented as S_1 ... S_n / S'




\subsection{Gentzen Sequents}

\begin{definition}[Gentzen Sequent] We define a \emph{Gentzen sequent} to be tuple $(V,E,G,L)$, where

\begin{itemize}

\item[$\blacktriangleright$] $V = \{x\}$ is a singleton;

\item[$\blacktriangleright$] $E = \emptyset$;

\item[$\blacktriangleright$] $G$ is a context-free grammar $\Lambda := \Gamma \vdash \Gamma$, $\Gamma ::= \phi \ | \ \Gamma , \Gamma$ where $\Gamma$ is generated by a context-free grammar;

\item[$\blacktriangleright$]  $L : V \mapsto \mathcal{L}(G)$, i.e. $L(x) \in \mathcal{L}(G)$.

\end{itemize}

\end{definition}




\subsection{Hypersequents}




\subsection{Linear Nested Sequents}





\subsection{Polylinear Nested Sequents}





\subsection{Nested Sequents}




\subsection{Display Sequents}





\subsection{Indexed-Nested Sequents}





\subsection{Labelled Sequents}




\subsection{General Relationships}


\begin{figure}
%\hspace{-5pt}{
\begin{center}
\resizebox{\columnwidth}{!}{
\begin{tabular}{c c} %@{\hskip -4em} c c}
\begin{tabular}{| c | c | c |} 
\hline
 \textbf{Sequent Type} & \textbf{Acronym} &  \textbf{Fundamental Graph}    \\
\hline
\hline
 Gentzen Sequent & $\gs$ &  Isolated Point \\
\hline
 Hypersequent & $\hs$ & Tree of Depth 1 \\
\hline
 Linear Nested Sequent & $\lns$ & Linear \\
\hline
 Polylinear Nested Sequent & $\plns$ & Polylinear \\
\hline
 Nested Sequent & $\ns$ & Tree  \\
\hline
 Display Sequent & $\ds$ & Polytree \\
\hline
 Indexed-Nested Sequent & $\ins$ & Directed Acyclic Graph \\
\hline
 Labelled Sequent & $\ls$ & Arbitrary Graph     \\
\hline
\end{tabular}

\begin{tabular}{c}
\begin{tikzpicture}
\node[] (GS) [] {$\gs$};
\node[] (LNS) [below=of GS, xshift=10mm,yshift=0mm] {$\lns$};
\node[] (PLNS) [right=of LNS, xshift=0mm,yshift=0mm] {$\plns$};
\node[] (HS) [below=of GS, xshift=-10mm,yshift=0mm] {$\hs$};
\node[] (NS) [below=of LNS, xshift=-10mm,yshift=0mm] {$\ns$};
\node[] (DS) [below=of NS, xshift=0mm,yshift=0mm] {$\ds$};
\node[] (INS) [right=of DS, xshift=0mm,yshift=0mm] {$\ins$};
\node[] (LS) [right=of INS, xshift=0mm,yshift=0mm] {$\ls$};


\path[->] (GS) edge[color=black] 
(LNS); 

\path[->] (GS) edge[color=black] 
(HS); 

\path[->] (LNS) edge[color=black] 
(PLNS); 

\path[->] (LNS) edge[color=black] 
(NS); 

\path[->] (PLNS) edge[color=black] 
(DS); 

\path[->] (HS) edge[color=black] 
(NS); 

\path[->] (NS) edge[color=black] 
(DS);

\path[->] (DS) edge[color=black] 
(INS); 

\path[->] (INS) edge[color=black] 
(LS);

%\path[->] (oiao) edge[color=black, bend right=10] 
%(oia); 

\end{tikzpicture}
\end{tabular}
\end{tabular}
}
\end{center}
%\hrule
\caption{Caption goes here}
\label{fig:hiearchy-of-calculi}
\end{figure}




==> refinement.tex <==

%NOTES: 
%(6) Give example with diamond rule and transitivity?
%(7) In each section give a table showing what rules are combined to make new propagation/reacability rules.
%(8) define length of (un)directed paths in each section





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%INTRODUCTION%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%NOTES:

%CITE: Pimentel 2018, Gore & Ramanayake 2014, Minari 2015?, LFCS2018, TOCL2020, LFCS2020, PRIMA2019


%\begin{comment}
\input{INTRO-refinement.tex}
%\end{comment}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%GRAMMAR LOGICS%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%NOTES:  (1) Refinement gives spearation property due to loss of converse rules! This useful in decidability (and perhaps other things--think about what else it could be useful for, i.e. conservativity?), (2) Define R_awu as inverse of R_\conv{a}uw so that we can do away with convers relational atoms, (3) Prove that converse rules can be eliminated, (4) Check that indeices start at 0 where necessary, (5) Does the separation property (used for conservativity) play any important role or use?, (6) Mention polytrees vs. trees and bring up interesting lemma where either R{a}wu or R{\conv{a}}uw can be used, (7) can explain how potentially can also get hp-admiss and hp-invert results by computing increase and decrease in size of proof when translating to parent labelled calculus, Maybe should mention that $D$ stands for `deep inference' here and in remamining section (i.e. next section), (8) Can add hypersequent section if so desired, (9) Define propagation graph in terms of sequent graph ot make more general and then can avoid repeating defintion in nested section and in FOInt section

%CITE: 

%\begin{comment}
\section{Refining Labelled Calculi for Grammar Logics}\label{SECT:Refine-Grammar}

\input{SEC-Refine-GramLog.tex}
%\end{comment}









%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%FO INTUITIONISTIC LOGIC%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%NOTES: (1) Separation property for bi-int (like for grammar logics), (2) Discuss reachability rules (point out how (forall left) and (exists right) are different from propagation rules

%CITE: 


%\begin{comment}
\section{Refining Labelled Calculi for First-Order Intuitionistic Logics}\label{SECT:Refine-FOInt}

\input{SEC-Refine-Int-FO.tex}
%\end{comment}









%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%DEONTIC STIT LOGICS%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%NOTES: (1) If hypersequent calculi or nested are discussed, then in previous sections may need to re-wrrite sentences about how nested will be observed in only Section 1 and 2 (without mention of this section: Section 3), (2) Mention the original propagation rule for D3? It is a new type

%CITE:


%\begin{comment}
\section{Refining Labelled Calculi for Deontic STIT Logics}\label{SECT:Refine-STIT}

\input{SEC-Refine-STIT.tex}
%\end{comment}









